A cluster of results on amplituhedron tiles

The amplituhedron is a mathematical object which was introduced to provide a geometric origin of scattering amplitudes in $\mathcal{N}=4$ super Yang Mills theory. It generalizes \emph{cyclic polytopes} and the \emph{positive Grassmannian}, and has a very rich combinatorics with connections to cluster algebras. In this article we provide a series of results about tiles and tilings of the $m=4$ amplituhedron. Firstly, we provide a full characterization of facets of BCFW tiles in terms of cluster variables for $\mbox{Gr}_{4,n}$. Secondly, we exhibit a tiling of the $m=4$ amplituhedron which involves a tile which does not come from the BCFW recurrence -- the \emph{spurion} tile, which also satisfies all cluster properties. Finally, strengthening the connection with cluster algebras, we show that each standard BCFW tile is the positive part of a cluster variety, which allows us to compute the canonical form of each such tile explicitly in terms of cluster variables for $\mbox{Gr}_{4,n}$. This paper is a companion to our previous paper ``Cluster algebras and tilings for the $m=4$ amplituhedron''.

==> variable_arrangements_figure.tex <==
%\scalebox{0.55}{
%\tiny
%\everydisplay{\fontsize{1}{1}\selectfont}
%\addtolength{\hoffset}{-4cm}
%\advance\hoffset by -4cm
%\begin{equation*}
    %\scalebox{0.45}{$
    %\begin{array}{cccccccccccccc}
    % R2L_T2B
    %\qR 4\times 1\\
                %&\qR1\times 1   &\qR1\times 2   &\qR\dots   &\qR1\times (n_R-4-1)         &\langle bcdn\rangle       &\langle acdn\rangle      &\langle cdn-ab-n12\rangle   &\qL1\times 1   &\qL1\times 2   &\qL\dots   &\qL1\times (n_L-4-2)   &\qL1\times (n_L-4-1)     &\langle 1cdn\rangle\\
                %&\langle abcn\rangle   &\qR2\times 1   &\qR\dots   &\qR2\times (n_R-4-2)   &\qR2\times (n_R-4-1)       &\qR(0\times 0)            &\qL4\times 1   &\qL2\times 1   &\qL2\times 2   &\qL\dots   &\qL2\times (n_L-4-2)   &\qL2\times (n_L-4-1)     &\langle 12dn\rangle\\
                %&\langle abcd\rangle   &\qR3\times 1   &\qR\dots   &\qR3\times (n_R-4-2)   &\qR3\times (n_R-4-1)   &\qR1\times (n_R-4)            &\qL4\times 2   &\qL3\times 1   &\qL3\times 2   &\qL\dots   &\qL3\times (n_L-4-2)   &\qL3\times (n_L-4-1)   &\qL1\times (n_L-4)\\
                %&\qR4\times 2   &\qR4\times 3   &\qR\dots     &\qR4\times (n_R-4)     &\qR3\times (n_R-4)   &\qR2\times (n_R-4)        &\langle a-1abb+1\rangle   &\qL4\times 3   &\qL4\times 4   &\qL\dots     &\qL4\times (n_L-4)     &\qL3\times (n_L-4)   &\qL2\times (n_L-4)%\\
            %\\  
    %% T2B_R2L
   %\qR 4\times 1&\\
                %&\langle abcn\rangle   &\qR1\times 1   &\qR\dots   &\qR1\times (n_R-4-2)         &\langle bcdn\rangle       &\langle acdn\rangle      &\langle cdn-ab-n12\rangle   &\qL1\times 1   &\qL1\times 2   &\qL\dots   &\qL1\times (n_L-4-2)   &\qL1\times (n_L-4-1)     &\langle 1cdn\rangle\\
                %&\langle abcd\rangle   &\qR2\times 1   &\qR\dots   &\qR2\times (n_R-4-2)   &\qR1\times (n_R-4-1)       &\qR(0\times 0)            &\qL4\times 1   &\qL2\times 1   &\qL2\times 2   &\qL\dots   &\qL2\times (n_L-4-2)   &\qL2\times (n_L-4-1)     &\langle 12dn\rangle\\
                %&\qR3\times 1   &\qR3\times 2   &\qR\dots   &\qR3\times (n_R-4-1)   &\qR2\times (n_R-4-1)   &\qR1\times (n_R-4)            &\qL4\times 2   &\qL3\times 1   &\qL3\times 2   &\qL\dots   &\qL3\times (n_L-4-2)   &\qL3\times (n_L-4-1)   &\qL1\times (n_L-4)\\
                %&\qR4\times 2   &\qR4\times 3   &\qR\dots     &\qR4\times (n_R-4)     &\qR3\times (n_R-4)   &\qR2\times (n_R-4)        &\langle a-1abb+1\rangle   &\qL4\times 3   &\qL4\times 4   &\qL\dots     &\qL4\times (n_L-4)     &\qL3\times (n_L-4)   &\qL2\times (n_L-4)
    %\end{array}
    %$}
    %\end{equation*}
%}
%\normalsize
%\begin{comment}
% {\fontsize{1}{3}\selectfont
% \begin{tikzpicture}[fill opacity=0.5,text opacity=1]
% % \begin{comment}
    
% %   \matrix{%\node[fill=red]{1};\\
  
% %     \node[fill=red]{$4\times1$};\\
% %                 &\node[fill=red]{$1\times1$};&\node[fill=red]{$1\times2$};&\node[fill=red]{$\dots$};&\node[fill=red]{$1\times(n_R-4-1)$};&\node{$\langle bcdn\rangle$};&\node{$\langle acdn\rangle$};&\node{$\langle cdn-ab-n12\rangle$};&\node[fill=blue]{$1\times1$};&\node[fill=blue]{$1\times2$};&\node[fill=blue]{$\dots$};&\node[fill=blue]{$1\times(n_L-4-2)$};&\node[fill=blue]{$1\times(n_L-4-1)$};&\node{$\langle 1cdn\rangle$};\\
% %                 &\node{$\langle abcn\rangle$};&\node[fill=red]{$2\times1$};&\node[fill=red]{$\dots$};&\node[fill=red]{$2\times(n_R-4-2)$};&\node[fill=red]{$2\times(n_R-4-1)$};&\node[fill=red]{$(0\times0)$};&\node[fill=blue]{$4\times1$};&\node[fill=blue]{$2\times1$};&\node[fill=blue]{$2\times2$};&\node[fill=blue]{$\dots$};&\node[fill=blue]{$2\times(n_L-4-2)$};&\node[fill=blue]{$2\times(n_L-4-1)$};&\node{$\langle 12dn\rangle$};\\
% %                 &\node{$\langle abcd\rangle$};&\node[fill=red]{$3\times1$};&\node[fill=red]{$\dots$};&\node[fill=red]{$3\times(n_R-4-2)$};&\node[fill=red]{$3\times(n_R-4-1)$};&\node[fill=red]{$1\times(n_R-4)$};&\node[fill=blue]{$4\times2$};&\node[fill=blue]{$3\times1$};&\node[fill=blue]{$3\times2$};&\node[fill=blue]{$\dots$};&\node[fill=blue]{$3\times(n_L-4-2)$};&\node[fill=blue]{$3\times(n_L-4-1)$};&\node[fill=blue]{$1\times(n_L-4)$};\\
% %                 &\node[fill=red]{$4\times2$};&\node[fill=red]{$4\times3$};&\node[fill=red]{$\dots$};&\node[fill=red]{$4\times(n_R-4)$};&\node[fill=red]{$3\times(n_R-4)$};&\node[fill=red]{$2\times(n_R-4)$};&\node{$\langle a-1abb+1\rangle$};&\node[fill=blue]{$4\times3$};&\node[fill=blue]{$4\times4$};&\node[fill=blue]{$\dots$};&\node[fill=blue]{$4\times(n_L-4)$};&\node[fill=blue]{$3\times(n_L-4)$};&\node[fill=blue]{$2\times(n_L-4)$};\\
% %   };
% % \end{comment}

%   \matrix{%\node[fill=red]{1};\\
  
%     \node{$4{\times1}$};\\
%                 &\node{$1{\times}1$};&\node{$1{\times}2$};&\node{$\dots$};&\node{$1{\times}(n_R{-}5)$};&\node{$\langle bcdn\rangle$};&\node{$\langle acdn\rangle$};&\node{$\langle cdn\br ab\br n12\rangle$};&\node{$1{\times}1$};&\node{$1{\times}2$};&\node{$\dots$};&\node{$1{\times}(n_L{-}6)$};&\node{$1{\times}(n_L{-}5)$};&\node{$\langle 1cdn\rangle$};\\
%                 &\node{$\langle abcn\rangle$};&\node{$2{\times}1$};&\node{$\dots$};&\node{$2{\times}(n_R{-}6)$};&\node{$2{\times}(n_R{-}5)$};&\node{$(0{\times}0)$};&\node{$4{\times}1$};&\node{$2{\times}1$};&\node{$2{\times}2$};&\node{$\dots$};&\node{$2{\times}(n_L{-}6)$};&\node{$2{\times}(n_L{-}5)$};&\node{$\langle 12dn\rangle$};\\
%                 &\node{$\langle abcd\rangle$};&\node{$3{\times}1$};&\node{$\dots$};&\node{$3{\times}(n_R{-}6)$};&\node{$3{\times}(n_R{-}5)$};&\node{$1{\times}(n_R{-}4)$};&\node{$4{\times}2$};&\node{$3{\times}1$};&\node{$3{\times}2$};&\node{$\dots$};&\node{$3{\times}(n_L{-}6)$};&\node{$3{\times}(n_L{-}5)$};&\node{$1{\times}(n_L{-}4)$};\\
%                 &\node{$4{\times}2$};&\node{$4{\times}3$};&\node{$\dots$};&\node{$4{\times}(n_R{-}4)$};&\node{$3{\times}(n_R{-}4)$};&\node{$2{\times}(n_R{-}4)$};&\node{$\langle a{-}1\,a\,b\,b{+}1\rangle$};&\node{$4{\times}3$};&\node{$4{\times}4$};&\node{$\dots$};&\node{$4{\times}(n_L{-}4)$};&\node{$3{\times}(n_L{-}4)$};&\node{$2{\times}(n_L{-}4)$};\\
%   };
%   %\fill[red] (-6,  -0.85)  rectangle (-0.45, 0.225);
%   %\fill[red] (-6.8,-0.85)  rectangle (-6,   -0.5);
%   %\fill[red] (-6.8, 0.225) rectangle (-3.3,  0.575);
%   %\fill[red] (-7.6, 0.575) rectangle (-6.8,  0.9);
  
%   %\fill[blue] (1.4,-0.85) rectangle (6.1, 0.575);
%   %\fill[blue] (0.1,-0.5)  rectangle (1.4, 0.225);
%   %\fill[blue] (6.1,-0.85) rectangle (7.6,-0.15);

%   \fill[red] (-7,0.575) rectangle (-6.3,0.9);
%   \fill[red] (-6.3,0.575) rectangle (-3,0.225);
%   \fill[red] (-5.5,0.225) rectangle (-0.45,-0.5);
%   \fill[red] (-6.3,-0.5) rectangle (-0.45,-0.85);

%   \fill[blue] (1.4,-0.85) rectangle (5.7, 0.575);
%   \fill[blue] (0.1,-0.5)  rectangle (1.4, 0.225);
%   \fill[blue] (5.7,-0.85) rectangle (7,-0.15);
% \end{tikzpicture}}

\vspace{10pt}
{\fontsize{1}{3}\selectfont
\begin{tikzpicture}[transform canvas={scale=0.75},fill opacity=0.5,text opacity=1]

  \matrix{
  
    \node{$\langle c' \,c \,d \,n\rangle$};\\
		&\node{$\langle a \,b\, c'\, n\rangle$};	&\node{$\langle a \,b\, c{-}2\, n\rangle$};	&\node{$\dots$};	&\node{$\langle a\, b\, b{+}2\, n\rangle$};	&\node{$\langle bcdn\rangle$};		&\node{$\langle acdn\rangle$};		&\node{$\langle cdn\br ab\br n12\rangle$};	&\node{$\langle 12an\rangle$};		&\node{$\langle 1 \,2 \,a{-}1\, n\rangle$};	&\node{$\dots$};	&\node{$\langle 125n\rangle$};	&\node{$\langle 124n\rangle$};	&\node{$\langle 1cdn\rangle$};\\
		&\node{$\langle abcn\rangle$};		&\node{$\langle a\, b\, c'\, c\rangle$};	&\node{$\dots$};	&\node{$\langle a\, b\, b{+}3\, b{+}4\rangle$};	&\node{$\langle a\, b\, b{+}2\, b{+}3\rangle$};	&\node{$\langle abdn\rangle$};		&\node{$\langle 1abn\rangle$};		&\node{$\langle 12ab\rangle$};		&\node{$\langle 1\, 2\, a{-}1\, a\rangle$};	&\node{$\dots$};	&\node{$\langle 1256\rangle$};	&\node{$\langle 1245\rangle$};	&\node{$\langle 12dn\rangle$};\\
		&\node{$\langle abcd\rangle$};		&\node{$\langle b\, c'\, c\, d\rangle$};	&\node{$\dots$};	&\node{$\langle b\, b{+}3\, b{+}4\, b{+}5\rangle$};	&\node{$\langle b\, b{+}2\, b{+}3\, b{+}4\rangle$};	&\node{$\langle a\, b\, b{+}1\, n\rangle$};	&\node{$\langle a{-}1\, a\, b\, n\rangle$};	&\node{$\langle 2abn\rangle$};		&\node{$\langle 2\, a{-}1\, a\, b\rangle$};	&\node{$\dots$};	&\node{$\langle 2567\rangle$};	&\node{$\langle 2456\rangle$};	&\node{$\langle 123n\rangle$};\\
		&\node{$\langle c{-}2\, c'\, c\, d\rangle$};	&\node{$\langle c{-}3\, c{-}2\, c'\, c\rangle$};	&\node{$\dots$};	&\node{$\langle a{-}2\, a{-}1\, a\, b\rangle$};	&\node{$\langle a{-}1\, a\, b\, b{+}1\rangle$};	&\node{$\langle a\, b\, b{+}1\, b{+}2\rangle$};	&\node{$\langle a{-}1\, a\, b\, b{+}1\rangle$};	&\node{$\langle a{-}2\, a{-}1\, a\, b\rangle$};	&\node{$\langle a{-}3\, a{-}2\, a{-}1\, a\rangle$};	&\node{$\dots$};	&\node{$\langle 3456\rangle$};	&\node{$\langle 2345\rangle$};	&\node{$\langle 1234\rangle$};\\
  };
  \fill[red] (-6.65,-0.85) rectangle (1,0.175);
  \fill[red] (-8.2,-0.85) rectangle (-6.65,-0.5);
  \fill[red] (-8.2,0.175) rectangle (-2.3,0.525);
  \fill[red] (-9.6,0.525) rectangle (-8.2,0.9);
  
  \fill[blue] (2.8,-0.85) rectangle (8.6,0.525);
  \fill[blue] (1.2,-0.5) rectangle (2.8,0.175);
  \fill[blue] (8.6,-0.85) rectangle (9.5,-0.15);
\end{tikzpicture}}

\vspace{10pt}
%\end{comment}
